TeV-scale bulk neutrino in warped extra-dimensions as a DM candidate

In this thesis, we have studied the possibility to identify one of the right-handed neutrinos entering the type-I seesaw mechanism as a Dark Matter (DM) candidate, within the warped extra-dimensions paradigm. As a first step, we have reviewed the existing literature on the Randall-Sundrum scenarios and the Goldberger-Wise stabilization mechanism. We have discussed a feasible realization of the type-I seesaw mechanism, implemented by warped compactification of an extra dimension. Taking advantage of recent studies, we have explored how the thermal DM can be included in the warped scenario. We have also outlined the current experimental bounds on the searches for DM and heavy Majorana neutrinos, as well as the theoretical constraints imposed. We have focused on generating a specific hierarchy between the right-handed neutrinos, that allows a correct realization of the seesaw while having an eV-scale sterile neutrino (that may be helpful to explain or soften the so-called "neutrino anomalies"), another one lying in the appropriate mass range for the DM and the last one sufficiently heavy to decouple. In our search of the parameter space, we found significant regions where this pattern can be realized. Moreover, we identified some problems that compromise the integrity of the model: it does not account for the measured masses and mixing of the light neutrino sector and, moreover, there exist some dangerous decay channels that prevents the DM candidate to be sufficiently stable. We discussed both problems and propose some reasonable solutions.

==> TeX_files/app-extradim-200429.tex <==
\chapter{Extra dimensional models}\label{Appendix A}

\section{Large Extra Dimensions}

At least, there are two fundamental energy scales in nature, the electroweak scale $m_{EW}\sim10^{3}$ GeV and the Planck scale $M_{Pl}=G_{N}^{-1/2}\sim10^{18}$ GeV. Explaining the hierarchy $m_{EW}/M_{Pl}\sim10^{-15}$ is one of the driving forces behind the construction of theories beyond the Standard Model.

\

We interpret $M_{Pl}$ as a fundamental scale under the assumption that gravity is unmodified between $\sim 1$ cm down to Planck length $\sim 10^{-33}$ cm, as gravitational forces have only been proven above that range. Questioning this extrapolation will lead to new physics beyond the SM.

\

Assuming that $m_{EW}$ is the only fundamental distance scale in nature will also set the strength of the gravitational interaction, we have to manage to obtain the usual $(1/M_{Pl})$. Suppose that there are $n$ extra compact spatial dimension of radius $\sim R$ (the spacetime will be $R^4\times M_n$, for $n\geq2$, and the volume of the n dimensional compact manifold is $\sim R^n$). The Planck scale of this theory is taken to be $M_{Pl(4+n)}\sim m_{EW}$. Applying Gauss law for the gravitational potential in $(4+n)$ dimensions will give us (for $r\gg R$):
\begin{equation}\label{1}
V(r)\sim \frac{m_1 m_2}{M_{Pl(4+n)}^{n+2} R^n} \frac{1}{r},
\end{equation}
so the effective 4D Planck constant results:
\begin{equation}\label{2}
M_{Pl}^2\sim M_{Pl(4+n)}^{2+n} R^n.
\end{equation}

For $n=2$ we will obtain $R\sim1$ mm, leading to deviations of Newtonian gravity below that distance. The effective 4 dimensional gravity is weakly coupled due to the large size $R$ of the extra dimensions, compared to the weak scale.

\

The SM particles can not freely propagate un the extra $n$ dimensions, must be localized to a 4 dimensional submanifold. As $m_{EW}$ is the only scale of the theory, the tickness of that manifold should be $\sim m_{EW}^{-1}$. The graviton is free to propagate in all $(4+n)$ dimensions.

\

The localization of the SM fields will be done trough trapping zero modes on topological defects. Our universe can be a 4 dimensional topological defect dynamically occurring in a higher-dimensional space. In this approach, particles can be viewed as zero modes trapped in the core of the defect. This is known as dynamical compactification.

\

This theory yields some experimental consequences independently of any specific realization:

\begin{enumerate}
	\item Gravity becomes comparable in strength to the gauge interactions at energies $m_{EW}\sim$ TeV. LHC could prove quantum gravity effects.
	\item In the case $n=2$, the gravitational force law should change from $1/r^2$ to $1/r^4$ on distances $\sim 1$ mm.
	\item In sufficiently hard collisions, of energy $\gtrsim m_{EW}$, the SM fields can acquire momentum in the extra dimensions and escape carrying away energy. This would put an upper limit to the transverse momentum at the LHC.
\end{enumerate}

While energy can be lost into the extra dimensions, electric charge (or any unbroken gauge charge) can not be lost because the photon is localized in our universe, and an isolated charge can not exist in the region where em field can not penetrate.

\section{Linear dilaton/Clockwork}

In the CW/LD scenario, we consider the metric:
\begin{equation}
\diff s^2=\mathrm{e}^{4/3 k r_c \phi} \eta_{\mu\nu} \diff x^\mu \diff x^\nu- r_c^2 \diff \phi^2,
\end{equation}
with the usual signature $\left(+,-,-,-,-\right)$ and greek indices running over 4 dimensions. As in the RS scenarios, the metric is non-factorizable, due to the warping factor $\mathrm{e}^{4/3 k r_c \phi}$. However, in the limit $k\rightarrow0$ we recover the flat LED case.

\

As before, the extra dimension is compactified on a $\mathcal{S}_1/\mathbb{Z}_2$ orbifold, with two branes located at the fixed points, $\phi=0,\pi$ (UV-brane and IR-brane respectively). In the following, we consider all SM and DM fields in the IR-brane, whereas in the UV-brane we can have any Planck-suppressed physics.

\

The 5-dimensional action is:
\begin{equation}
S=S_{bulk}+S_{IR}+S_{UV},
\end{equation}
where we can explicitly write these terms as:
\begin{equation}
\begin{split}
S_{bulk}&=\frac{M_{5}^3}{2}\int \diff^4x\int^{\pi}_{0} r_c \diff \phi \sqrt{\vphantom{G}^{(5)}G} \ \mathrm{e}^{\mathcal{S}} \left[\vphantom{R}^{(5)}R+\vphantom{G}^{(5)}G^{MN}\partial_M \mathcal{S}\partial_N \mathcal{S}+4k^2\right],\\
S_{IR}&=\int \diff^4x \sqrt{-g} \left[\lag_{SM}+\lag_{DM}-f_{IR}^4\right],\\
S_{UV}&=\int \diff^4x \sqrt{-g} \left[-f_{UV}^4+...\right],
\end{split}
\end{equation}
where $\vphantom{G}^{(5)}G_{MN}$ and $\vphantom{R}^{(5)}R$ are the 5-dimensional metric and Ricci scalar, $\mathcal{S}$ is the dilaton field, $\mathcal{S}=2k r_c \phi$, and $f_{IR}$, $f_{UV}$ are the brane tensions for the two branes.

==> TeX_files/app-lorentz-190529.tex <==
\chapter{The Lorentz Group}\label{Appendix F}

The postulates of Special Relativity tells that the velocity of light \textit{c} is the same in all inertial frames. If in one frame we have a light signal at space-time point $(t,x_i)$ and in another frame we found it at $(t',x'_i)$, the previous restriction implies:
%
\begin{equation}\label{F.1}
s^2\equiv c^2 t^2 - x_i x_i=c^2 t'^2 - x'_i x'_i.
\end{equation}

Choosing units such that $c=1$ and adopting the contracted notation $x^\mu$, $\mu=0,1,2,3$ with $x^0=t$ and $(x^1,x^2,x^3)=\vec{x}$, $s^2$ may be written as:
%
\begin{equation}\label{F.2}
s^2\equiv x^\mu x^\nu g_{\mu \nu}=x'^\mu x'^\nu g_{\mu \nu},
\end{equation}

where the metric $g_{\mu \nu}$ is zero except for $\mu=\nu$ when $g_{00}=-g_{11}=-g_{22}=-g_{33}=1$

\

Now we look for a linear transformation which preserves $s^2$:
%
\begin{equation}\label{F.3}
x'^{\mu}=\Lambda^{\mu}_{\nu} x^{\nu}.
\end{equation}

It must satisfy:
%
\begin{equation}\label{F.4}
x'^\mu x'^\nu g_{\mu \nu}=\Lambda^{\mu}_{\rho} x^{\rho} \Lambda^{\nu}_{\sigma} x^{\sigma} g_{\mu \nu}=x^{\rho} x^{\sigma} g_{\rho \sigma}.
\end{equation}

Because that must be hold by every $x^{\mu}$, we conclude:
%
\begin{equation}\label{F.5}
g_{\rho \sigma}=g_{\mu \nu} \Lambda^{\mu}_{\rho} \Lambda^{\nu}_{\sigma}.
\end{equation}

One may show that these transformations satisfy the group axioms.

\

If we use matrix notation, regarding $x^{\mu}$ as a column vector $x$, the metric as a squared matrix $g$ and the transformation as the matrix equivalent off the coefficients $L$, we can rewrite the previous relation as:
%
\begin{equation}\label{F.6}
g=L^tgL.
\end{equation}

We must point out two consequences of the above discussion. First, if we take the determinant in the last equation:
%
\begin{equation}\label{F.7}
\det{g}=\det{L^t} \det{g} \det{L},
\end{equation}

from which we deduce:
%
\begin{equation}\label{F.8}
\det{L}=\pm 1.
\end{equation}

Second, taking the $00$ entry in equation (5):
%
\begin{equation}\label{F.9}
1=g_{\mu \nu} \Lambda^{\mu}_{0} \Lambda^{\nu}_{0}=\left(\Lambda^{0}_{0}\right)^2-\left(\Lambda^{i}_{i}\right)^2,
\end{equation}
%
shows that:
%
\begin{equation}\label{F.10}
\left|\Lambda^{0}_{0}\right| \geq 1.
\end{equation}

Any Lorentz transformation can be decomposed as the product of rotations, boost transformations, time inversion and full inversion. Consider the infinitesimal Lorentz Transformation:
%
\begin{equation}\label{F.11}
\Lambda^{\mu}_{\nu}=\delta^{\mu}_{\nu} + \varepsilon^{\mu}_{\nu}.
\end{equation}

Evaluating (\ref{F.5}) to first order in $\epsilon$ gives:
%
\begin{equation}\label{F.12}
g_{\rho \sigma}=g_{\rho \sigma} + g_{\rho \nu} \varepsilon^{\nu}_{\sigma} + g_{\mu \sigma} \varepsilon^{\mu}_{\rho},
\end{equation}
%
which is equivalnet to:
%
\begin{equation}\label{F.13}
g_{\nu \rho} \varepsilon^{\rho}_{\mu} + g_{\mu \rho} \varepsilon^{\rho}_{\nu}=0.
\end{equation}

Since the metric can low indices, that equation becomes:
%
\begin{equation}\label{F.14}
\varepsilon_{\nu \mu} + \varepsilon_{\mu \nu}=0
\end{equation}

That is, $\varepsilon_{\mu \nu}$ is an antisymmetric tensor with only 6 independent entries. It could be advertised, since there's three boosts and three rotations, one for each space direction.

\

We can introduce the Hermitian generators:
%
\begin{equation}\label{F.15}
L_{\mu \nu}\equiv\imath \left(x_{\mu} \partial_{\nu}-x_{\nu} \partial_{\mu}\right).
\end{equation}

The $L_{\mu \nu}$'s satisfy the Lie algebra of $SO(3,1)$:
%
\begin{equation}\label{F.16}
\left[L_{\mu \nu},L_{\rho \sigma}\right] = \imath g_{\nu \rho} L_{\mu \sigma} - \imath g_{\mu \rho} L_{\nu \sigma} - \imath g_{\nu \sigma} L_{\mu \rho} + \imath g_{\mu \sigma} L_{\nu \rho}.
\end{equation}

The most general representation of the generators of $SO(3,1)$ obeying that commutation relation is given by:
%
\begin{equation}\label{F.17}
M_{\mu \nu}\equiv \imath \left(x_{\mu} \partial_{\nu}-x_{\nu} \partial_{\mu}\right) + S_{\mu \nu},
\end{equation}
%
where the Hermitian operator $S_{\mu \nu}$ commute with $L_{\mu \nu}$ and satisfy the same Lie algebra. These generators form an algebra among themselves:
%
\begin{equation}\label{F.18}
\left[M_{i j},M_{k l}\right] = -\imath \delta_{j k} M_{i l} + \imath \delta_{i k} M_{j l} + \imath \delta_{j l} M_{i k} - \imath \delta_{i l} M_{j k},
\end{equation}
%
which is that of the rotation group $SU(2)$. If we introduce the operators:
%
\begin{equation}\label{F.19}
J_i\equiv\frac{1}{2} \ \epsilon_{ijk} M_{jk},
\end{equation}
%
\begin{equation}\label{F.20}
K_i\equiv M_{0i},
\end{equation}
%
where $\epsilon_{ijk}$ is the Levi-Civita symbol, the next commutation relations follows:
%
\begin{equation}\label{F.21}
\left[J_i,J_j\right]=\imath \epsilon_{ijk} J_k,
\end{equation}
%
\begin{equation}\label{F.22}
\left[K_i,K_j\right]=-\imath \epsilon_{ijk} J_k,
\end{equation}
%
\begin{equation}\label{F.23}
\left[J_i,K_j\right]=\imath \epsilon_{ijk} K_k.
\end{equation}

These relations may be disentangled by introducing the linear combination:
%
\begin{equation}\label{F.24}
N_i\equiv \frac{1}{2} \ \left( J_i + \imath K_i\right).
\end{equation}

Although it's not Hermitian, it yield simple commutation relations:
%
\begin{equation}\label{F.25}
\left[N_i,N_j^\dagger\right]=0,
\end{equation}
%
\begin{equation}\label{F.26}
\left[N_i,N_j\right]=\imath \epsilon_{ijk} N_k,
\end{equation}
%
\begin{equation}\label{F.27}
\left[N_i^\dagger,N_j^\dagger\right]=\imath \epsilon_{ijk} N_k^\dagger.
\end{equation}

==> TeX_files/bib-200508.tex <==
\begin{thebibliography}{9}
\addcontentsline{toc}{chapter}{Bibliography}
	
\bibitem{led1}
N. Arkani-Hamed, S. Dimopoulos and G. Dvali, \textit{The Hierarchy Problem and New Dimensions at a Millimeter}, \href{https://doi.org/10.1016/S0370-2693(98)00466-3}{\textit{Phys. Lett.} \textbf{B436} (1998) 257–263}, [\href{https://arxiv.org/abs/hep-ph/9803315}{hep-ph/9803315}].

\bibitem{dynamical}
G. Dvali and M. Shifman (1996). Dynamical Compactification as a Mechanism of Spontaneous Supersymmetry Breaking. \url{hep-th/9611213}.

\bibitem{led2}
I. Antoniadis, N. Arkani-Hamed, S. Dimopoulos and G. Dvali, \textit{New dimensions at a millimeter to a Fermi and superstrings at a TeV}, \href{https://doi.org/10.1016/S0370-2693(98)00860-0}{\textit{Phys. Lett.} \textbf{B436} (1998) 257–263}, [\href{https://arxiv.org/abs/hep-ph/9804398}{hep-ph/9804398}].

\bibitem{rs1}
L. Randall and R. Sundrum, \textit{A Large Mass Hierarchy from a Small Extra Dimension}, \href{https://doi.org/10.1103/PhysRevLett.83.3370}{\textit{Phys. Rev. Lett.} \textbf{83} (1999) 3370–3373}, [\href{https://arxiv.org/abs/hep-ph/9905221}{hep-ph/9905221}].

\bibitem{rs2}
L. Randall and R. Sundrum, \textit{An Alternative to Compactification}, \href{https://doi.org/10.1103/PhysRevLett.83.4690}{\textit{Phys. Rev. Lett.} \textbf{83}
(1999) 4690–4693}, [\href{https://arxiv.org/abs/hep-th/9906064}{hep-th/9906064}].

\bibitem{cw1}
G. Giudice and M. McCullough, \textit{A Clockwork Theory}, \href{https://doi.org/10.1007/JHEP02(2017)036}{\textit{JHEP} \textbf{02} (2017) 036}, [\href{https://arxiv.org/abs/1610.07962}{1610.07962}].

\bibitem{cw2}
G. Giudice, Y. Kats, M. McCullough, R. Torre and A. Urbano, \textit{Clockwork/Linear Dilaton: Structure and Phenomenology}, \href{https://doi.org/10.1007/JHEP06(2018)009}{\textit{JHEP} \textbf{06} (2018) 009}, [\href{https://arxiv.org/abs/1711.08437}{1711.08437}].

\bibitem{ific1}
M. Folgado, A. Donini and N. Rius,\textit{ Gravity-mediated Scalar Dark Matter in Warped Extra-Dimensions}, [\href{https://arxiv.org/abs/1907.04340}{1907.04340}].

\bibitem{ific2}
M. Folgado, A. Donini and N. Rius, \textit{Gravity-mediated Dark Matter in Clockwork/Linear Dilaton Extra-Dimensions}, [\href{https://arxiv.org/abs/1912.02689}{1912.02689}].

\bibitem{ific3}
M. Folgado, A. Donini and N. Rius, \textit{Spin-dependence of Gravity-mediated Dark Matter in Warped Extra-Dimensions}, Manuscript in preparation.

\bibitem{pheno1}
H. Lee, M. Park and V. Sanz, \textit{Gravity-mediated (or Composite) Dark Matter}, \href{https://doi.org/10.1140/epjc/s10052-014-2715-8}{\textit{Eur. Phys. J.} \textbf{C74} (2014) 2715}, [\href{https://arxiv.org/abs/1306.4107}{1306.4107}].

\bibitem{pheno2}
S. Kawai and N. Okada (2020). eV-scale sterile neutrinos from an extra dimension. \url{hep-ph/1910.02936}

\bibitem{pheno3}
T. Gherghetta and A. Pomarol (2000). Bulk fields and supersymmetry in a slice of AdS. \url{hep-ph/0003129}

\bibitem{pheno4}
Y. Grossman and M. Neubert (1999). Neutrino masses and mixings in non-factorizable geometry. \url{hep-ph/9912408}

\bibitem{pheno5}
S. Chang, J. Hisano, H. Nakano, N. Okada nd M. Yamaguchi (1999). Bulk Standard Model in the Randall-Sundrum Background. \url{hep-ph/9912498}

\bibitem{pheno6}
H. Davoudiasl, J. Hewett and T. Rizzo (1999). Warped Phenomenology. \url{hep-ph/9909255}

\bibitem{velexp}
P. Gondolo and G. Gelmini, \textit{Cosmic abundances of stable particles: Improved analysis}, \href{https://doi.org/10.1016/0550-3213(91)90438-4}{\textit{Nucl. Phys.} \textbf{B360} (1991) 145–179}.

\bibitem{majoranarules}
H. Eck, O. Hahn and J. Küblbeck, \textit{Compact Feynman rules for Majorana fermions}, \href{https://doi.org/10.1016/0370-2693(92)91045-B}{\textit{Phys. Lett.} \textbf{B291} (1992) 278–280}.
\end{thebibliography}
